Large-Scale Object Detection of Images from Network Cameras in Variable Ambient Lighting Conditions

Computer vision relies on labeled datasets for training and evaluation in detecting and recognizing objects. The popular computer vision program, YOLO ("You Only Look Once"), has been shown to accurately detect objects in many major image datasets. However, the images found in those datasets, are independent of one another and cannot be used to test YOLO's consistency at detecting the same object as its environment (e.g. ambient lighting) changes. This paper describes a novel effort to evaluate YOLO's consistency for large-scale applications. It does so by working (a) at large scale and (b) by using consecutive images from a curated network of public video cameras deployed in a variety of real-world situations, including traffic intersections, national parks, shopping malls, university campuses, etc. We specifically examine YOLO's ability to detect objects in different scenarios (e.g., daytime vs. night), leveraging the cameras' ability to rapidly retrieve many successive images for evaluating detection consistency. Using our camera network and advanced computing resources (supercomputers), we analyzed more than 5 million images captured by 140 network cameras in 24 hours. Compared with labels marked by humans (considered as "ground truth"), YOLO struggles to consistently detect the same humans and cars as their positions change from one frame to the next; it also struggles to detect objects at night time. Our findings suggest that state-of-the art vision solutions should be trained by data from network camera with contextual information before they can be deployed in applications that demand high consistency on object detection.

==> oldabstract.tex <==

\input{settings}
\begin{comment}
\end{comment}

\title{Large-Scale Objection Detection of Images from Network Cameras}

\author{Caleb Tung, Matthew R. Kelleher, Ryan J. Schlueter, Binhan Xu, Yung-Hsiang Lu \\
\small \{tung3, kellehem, rschluet, xu938, yunglu\}@purdue.edu \\
School of Electrical and Computer Engineering \\
Purdue University, West Lafayette, IN, USA \\
George K. Thiruvathukal \\
gkt@cs.luc.edu \\
Department of Computer Science \\
Loyola University Chicago, Chicago, IL, USA}


\date{}

\begin{document}
\maketitle


\todo{Please add the authors' affiliations and their email addresses}

\todo{Change format to IEEE double-column format before submitting}

\input{abstract}



\section{Introduction}

Your introduction goes here! Some examples of commonly used commands and features are listed below, to help you get started. If you have a question, please use the help menu (``?'') on the top bar to search for help or ask us a question. 

\section{Some examples to get started}

\subsection{How to include Figures}

First you have to upload the image file from your computer using the upload link the project menu. Then use the includegraphics command to include it in your document. Use the figure environment and the caption command to add a number and a caption to your figure. See the code for Figure \ref{fig:frog} in this section for an example.

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{frog.jpg}
\caption{\label{fig:frog}This frog was uploaded via the project menu.}
\end{figure}

\subsection{How to add Comments}

Comments can be added to your project by clicking on the comment icon in the toolbar above. % * <john.hammersley@gmail.com> 2016-07-03T09:54:16.211Z:
%
% Here's an example comment!
%
To reply to a comment, simply click the reply button in the lower right corner of the comment, and you can close them when you're done.

Comments can also be added to the margins of the compiled PDF using the todo command\todo{Here's a comment in the margin!}, as shown in the example on the right. You can also add inline comments:

\todo[inline, color=green!40]{This is an inline comment.}

\subsection{How to add Tables}

Use the table and tabular commands for basic tables --- see Table~\ref{tab:widgets}, for example. 

\begin{table}
\centering
\begin{tabular}{l|r}
Item & Quantity \\\hline
Widgets & 42 \\
Gadgets & 13
\end{tabular}
\caption{\label{tab:widgets}An example table.}
\end{table}

\subsection{How to write Mathematics}

\LaTeX{} is great at typesetting mathematics. Let $X_1, X_2, \ldots, X_n$ be a sequence of independent and identically distributed random variables with $\text{E}[X_i] = \mu$ and $\text{Var}[X_i] = \sigma^2 < \infty$, and let
\[S_n = \frac{X_1 + X_2 + \cdots + X_n}{n}
      = \frac{1}{n}\sum_{i}^{n} X_i\]
denote their mean. Then as $n$ approaches infinity, the random variables $\sqrt{n}(S_n - \mu)$ converge in distribution to a normal $\mathcal{N}(0, \sigma^2)$.


\subsection{How to create Sections and Subsections}

Use section and subsections to organize your document. Simply use the section and subsection buttons in the toolbar to create them, and we'll handle all the formatting and numbering automatically.

\subsection{How to add Lists}

You can make lists with automatic numbering \dots

\begin{enumerate}
\item Like this,
\item and like this.
\end{enumerate}
\dots or bullet points \dots
\begin{itemize}
\item Like this,
\item and like this.
\end{itemize}

\subsection{How to add Citations and a References List}

You can upload a \verb|.bib| file containing your BibTeX entries, created with JabRef; or import your \href{https://www.overleaf.com/blog/184}{Mendeley}, CiteULike or Zotero library as a \verb|.bib| file. You can then cite entries from it, like this: \cite{greenwade93}. Just remember to specify a bibliography style, as well as the filename of the \verb|.bib|.

You can find a \href{https://www.overleaf.com/help/97-how-to-include-a-bibliography-using-bibtex}{video tutorial here} to learn more about BibTeX.

We hope you find Overleaf useful, and please let us know if you have any feedback using the help menu above --- or use the contact form at \url{https://www.overleaf.com/contact}!

\bibliographystyle{alpha}
\bibliography{sample}

\end{document}

==> unused.tex <==

\subsection{Smaller-scale VS large scale object detection}
{\bf Give the relevance+importance of object detection in computer vision applications with examples}



Modern camera-based computer vision technologies often rely heavily on object detection. Cars with collision avoidance systems analyze car-mounted camera images for the presence of pedestrians or other cars, then respond by appropriately applying brakes~\cite{Eyesight_page}. Smartphone apps employ object detection to identify the locations of human faces in a photo and blur them out for privacy~\cite{Snapchat_patent}.

{\bf Note the limitations of the image data being processed by those smaller, more focused applications}
Computer vision applications like the ones described above rely on a small number of cameras looking at specific scene types (a view of the road, images of human faces, in the above respective cases).

{\bf Contrast with the huge range of image data from indoor/outdoor network cameras}
In contrast, the type of image data retrieved from indoor/outdoor network cameras varies significantly based on the camera's changing immediate environment~\cite{IRI_paper}. Not only do the subjects of the camera change (\textit{e.g.} a traffic camera frame contains more cars during rush hour than at 3 A.M.)~\cite{IRI_paper}, but the quality of the images could change as well. Overcast weather could cause gray-colored objects to blend into the background. At nighttime, the glare of neon lights and illuminated billboards could worsen change the appearance of objects in the frame.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=\linewidth]{dublin-day-night}
  \caption{A Dublin, Ireland outdoor network camera experiences significant environment changes throughout the day}\label{fig:dublin-day-night}
\end{figure}

Given that changing environmental factors affect human vision (which is used to define the "ground truth" for computer vision), it stands to reason that the accuracy performance of computer vision programs would be affected by those factors as well.

{\bf Stress that object detectors need to be able to deal with this wide range of data if we are to go large-scale}
In order to use object detectors like YOLO on images streamed from a large number of network cameras placed around the world, then, the object detectors must be able to cope with the myriad effects of the changing camera environments and locales. To that end, we wish to evaluate YOLO out-of-the-box for its ability to perform with this kind of varying data.

\subsection{The YOLO object detector at large scale}
{\bf Discuss YOLO has been evaluated with more focused image datasets}
YOLO is considered to be state-of-the-art~\cite{Traffic_Light_paper}. Redmon, \textit{et al.} tested YOLO and found that it outperformed several of its object detection contemporaries such as Single-Shot Detector in terms of both accuracy and speed~\cite{YOLO_site,SSD_paper,YOLO_paper}.  However, their test was run against the COCO (``Common Object in Context'')~\cite{COCO_paper} and PASCAL VOC (``Pattern Analysis, Statistical Modeling, and Computational Learning Visual Object Classes'')~\cite{PascalVOC_paper} image datasets~\cite{YOLO_paper}, neither of which accounts for contextual information such as location, nighttime VS daytime, weather, etc.

{\bf Since YOLO has been used as the object detector of choice for many applications, we choose to test it for our large-scale project--additionally, those applications are not at all like a large-scale network camera analyzer}
In addition, YOLO is employed in many computer vision applications with varying data, which suggests that it may be a good candidate for large-scale network camera object detection. Jensen, \textit{et al.} successfully used YOLO as a stoplight detector for autonomous vehicles~\cite{Traffic_Light_paper}. Al-masni, \textit{et al.} designed a YOLO-based malignant tumor deep learning model for breast cancer detection~\cite{BreastCancer_paper}. Xie, \textit{et al.} developed a prototype multi-directional YOLO license plate detector~\cite{LicensePlate_paper}. In all of these cases, however, the image data was very focused and did not contain the amounts of variation introduced by outdoor/indoor network cameras.

\subsection{Paper outline}
{\bf Describe the knowledge this paper adds to the field}
Our paper examines how well YOLO maintains its detection accuracy out-of-the-box while processing images from a collection of many network cameras from around the globe. Further, it discusses the implications of these findings for large-scale network camera analysis.

{\bf Organization of paper}
The rest of this paper is organized as follows. In Section II, we outline our procedure for observing the accuracy of YOLO during large-scale object detection.  Section III describes the recorded accuracy performance of YOLO on a selection of changing factors.  Finally, the paper is concluded in Section IV with a discussion of the results and what they mean for large-scale object detection


YOLO obtains fast framerates on high-powered computers~\cite{YOLO_paper}. Therefore, in order to test YOLO at a large scale, we ran YOLO using two supercomputing clusters: Intel Corporation's ``vLab'' Academic Cluster~\cite{IntelvLab_page} and Argonne National Laboratory's ``Cooley'' compute cluster~\cite{Cooley_page}.

\todo[inline]{\textbf{CT: I did not mention KNM, just in case that violates the Intel agreement}}
\textbf{vLab} is a supercomputing cluster maintained by the Intel Corporation. The cluster consists of over 200 nodes. Each node runs an Intel cluster CPU--the CPUs include ``Skylake'' ~\cite{Skylake_page} and ``Knights Landing''~\cite{KnightsLanding_page} Xeon Phi cores. The cluster features few GPUs--it features specially CPU-optimized versions of software packages like Python and Caffe and is designed for machine learning research. Each node packs 220 GB of RAM and a 400 GB solid state drive. A 10Gbps network connection ties the entire cluster into the central 2PB file storage system. Users submit jobs using the PBS scheduler on vLab.

\textbf{Cooley} is a supercomputing cluster based at Argonne National Laboratory. With 128 nodes total (126 usable for user jobs), it is primarily intended to support visualization applications. However, it is a powerful computer for development and testing purposes. Each node has 12 CPU cores and one NVIDIA Tesla K80 dual-GPU card.  Aggregate GPU peak performance is over 293 teraflops double precision (using base GPU clocks), and the entire system has a total of 47 terabytes of system RAM and 3 terabytes of GPU RAM.  Users must use a job scheduler (Cobalt) to submit and run jobs on the Argonne Cooley cluster.

On Cooley, YOLO ran on its original ``Darknet'' neural net framework~\cite{YOLO_site}, leveraging the compute nodes' onboard NVIDIA GPUs to process quickly. On vLab, we used a build of YOLO that ran on Intel-Caffe~\cite{IntelNervana_page}, an Intel-optimized fork of the Caffe neural net framework~\cite{IntelNervana_page}. Speed was further optimized by Intel's Math Kernel Library~\cite{IntelNervana_page}, thus allowing YOLO to run usably quickly on Intel's CPUs. Both compute clusters were equipped with hundreds of terabytes of storage which accommodated the space consumed by the images from the CAM\textsuperscript{2} cameras.

\todo[inline]{Caleb: Please mimic the above paragraphs to describe the INtel cluster.}


\subsection{Experiment Procedure}
Before running YOLO, we collected approximately 5 million unique images from a set of 140 CAM\textsuperscript{2}'s highest quality cameras (roughly 30 frames-per-second (FPS) streaming, 480p-720p resolution) placed in the United States and Europe. These images were collected from the cameras at at regular intervals through a period of 24 hours. The images were then stashed on the network filesystems of the vLab and Cooley clusters. Finally, YOLO was run on those 5 million images, and it's detection result labels (labels are bounding boxes for humans and cars) were saved. We only kept the labels if YOLO's confidence score (a measure of how accurate it believed a given label to be) was higher than 0.3.

\subsection{Interpretation of Detection Results}
In order to find areas where YOLO had trouble with the large-scale network camera data, we needed to hand-label the people and cars in the images to compare with YOLO's labels. Hand labels are considered as ground truth because they are created based on human vision. However, given that it would be far too time-consuming to hand-label 5 million images, we devised this method for sampling our data:

\begin{enumerate}
\item 4 images were uniformly sampled from each of the 140 cameras at hourly intervals, over the 24-hour period. Thus, we would have images from all cameras spanning a full day. In total, we sampled over 13,000 unique images to be reviewed for data integrity.
\item The 13,000 images were manually reviewed for any evidence of corruption or other strange potential artifacts of the livestreaming process. Once the images were determined to be clean, the reviewers looked for either humans or cars in the data. If either subject appeared in an image, that image's source camera was flagged for final analysis.
\item From every camera flagged for final analysis, we selected one clean image from each of the 24 hours to be carefully hand-labeled as ground truth.
\end{enumerate}

Finally, we evaluated YOLO's labels against our ground-truth labels. The closer YOLO's label was to a ground-truth label, the more accurate the detection. We used a method called "Intersection over Union" (IOU) of bounding boxes to measure the accuracy.  Suppose $B_1$ is the bounding box marked by a vision program
and $B_2$ is the bounding box marked by a person.  IOU is defined as

\begin{equation*}
  \text{IOU} = \frac{B_1 \cap B_2}{B_1 \cup B_2}. 
\end{equation*}

A\textsubscript{I} is the area covered by the intersection of YOLO's bounding box and the ground-truth bounding box. A\textsubscript{U} is the area covered by the union between those two bounding boxes. Thus, the closer BBIOU is to 1.0, the more similar the two bounding boxes are, and by extension, the more accurate YOLO's detection is.

Our evaluation consisted of the following:

\begin{itemize}
\item Investigating whether YOLO can make accurate detections when the camera is far away from its subject
\item Examining how YOLO's accuracy changed as the time changed from day to night
\item Investigating whether motion blur has an impact on YOLO's accuracy
\item Identifying situations in which YOLO detected an object when it should not have
\end{itemize}





